Harmony in Diversity: Merging Neural Networks with Canonical Correlation Analysis

Combining the predictions of multiple trained models through ensembling is generally a good way to improve accuracy by leveraging the different learned features of the models, however it comes with high computational and storage costs. Model fusion, the act of merging multiple models into one by combining their parameters reduces these costs but doesn't work as well in practice. Indeed, neural network loss landscapes are high-dimensional and non-convex and the minima found through learning are typically separated by high loss barriers. Numerous recent works have been focused on finding permutations matching one network features to the features of a second one, lowering the loss barrier on the linear path between them in parameter space. However, permutations are restrictive since they assume a one-to-one mapping between the different models' neurons exists. We propose a new model merging algorithm, CCA Merge, which is based on Canonical Correlation Analysis and aims to maximize the correlations between linear combinations of the model features. We show that our alignment method leads to better performances than past methods when averaging models trained on the same, or differing data splits. We also extend this analysis into the harder setting where more than 2 models are merged, and we find that CCA Merge works significantly better than past methods. Our code is publicly available at https://github.com/shoroi/align-n-merge

==> archive/s2_related_work.tex <==
\vspace{-10pt}
\section{Related Work}\label{s:related_work}
\vspace{-5pt}
\paragraph{Mode connectivity}
\cite{freeman2017topology} proved theoretically that one-layered ReLU neural networks have asymptotically connected level sets, i.e. as the number of neurons increases two minima of such a network are connected by a low loss path in parameter space. \cite{garipov2018_fge} and \cite{draxler2018_no-barriers} explore these ideas empirically and introduce the concept of \emph{mode connectivity} to describe ANN minima that are connected by nonlinear paths in parameter space along which the loss remains low, the maximum of the loss along this path was termed the \emph{energy barrier}, and both works proposed algorithms for finding such paths. \cite{garipov2018_fge} further proposed \emph{Fast Geometric Ensembling} (FGE) as a way to take advantage of mode connectivity by ensembling multiple model checkpoints from a single training trajectory. 
%
\cite{pmlr-v119-frankle20a_lmc_lth} introduced the concept of \emph{linear mode connectivity} which describes the scenario in which two ANN minima are connected by a \emph{linear} low loss path in parameter space. They used linear mode connectivity to study network stability to SGD noise (i.e. different data orders and augmentations). They found that at initialization, networks are typically not stable, i.e. training with different SGD noise from a random initialization typically leads to optima that are not linearly mode connected, however early in training models become stable to such noise.
\vspace{-5pt}
\paragraph{Model merging}
More recently, \cite{entezari2022_perm-invariance-lmc} have conjectured that ``Most SGD solutions belong to a set $\mathcal{S}$ whose elements can be permuted in such a way that there is no barrier on the linear interpolation between any two permuted elements in $\mathcal{S}$'' or in other words most SGD solutions are linearly mode connected provided the right permutation is applied to align the two solutions. They then perform experiments that support this conjecture and also empirically establish that increasing network width, decreasing depth, using more expressive architectures, or training on a simpler task all help linear mode connectivity by decreasing the loss barrier between two optima. Many other works seem to support this conjecture. For example, \cite{singh-jaggi2020_OT-fusion} and \cite{pena2023_sinkhorn-rebasin} propose optimal transport-based methods for finding the best transformation to match two models.
%The method of \cite{pena2023_sinkhorn-rebasin} is differentiable and they relax the constraint of finding a binary permutation matrix but add an entropy regularizer instead. 
%
\cite{ainsworth2023_git-rebasin} propose an algorithm for finding the optimal permutation for merging models based on the distances between the weights of the models themselves. \cite{jordan2023repair} exposes the phenomenon in which interpolated deep networks suffer a variance collapse in their activations leading to poor performance. They propose REPAIR which mitigates this problem by rescaling the preactivations of interpolated networks through the recomputation of BatchNorm statistics. 
\vspace{-5pt}
\paragraph{``Easy'' settings for model averaging} Linear mode connectivity is hard to achieve in deep learning models. \cite{pmlr-v119-frankle20a_lmc_lth} established that even models being trained on the same dataset with the same learning procedure and even the same initialization might not be linearly mode connected if they have different data orders/augmentations.
%
It seems that only models that are already very close in parameter space can be directly combined through linear interpolation. This is the case for snapshots of a model taken at different points during its training trajectory \citep{garipov2018_fge, izmailov2018_averaging} or multiple fine-tuned models with the same pre-trained initialization \citep{wortsman22_modelsoups, ilharco2023_task-arithmetic, yadav2023tiesmerging}. This latter setting is the one typically considered in NLP research. Another setting that is worth mentioning here is the ``federated learning'' inspired one where models are merged every couple of epochs during training \citep{jolicoeurmartineau2023_papa}. The common starting point in parameter space and the small number of training iterations before merging make LMC easier to attain.

We emphasize that these settings are different from ours in which we aim to merge \emph{fully trained models} with different parameter initializations and SGD noise (data order and augmentations).
\vspace{-5pt}
\paragraph{Merging multiple models}
Merging more than two models has only been explored thoroughly in the ``easy'' settings stated above. For example \cite{wortsman22_modelsoups} averages models fine-tuned with different hyperparameter configurations and finds that this improves accuracy and robustness. \cite{jolicoeurmartineau2023_papa} averages the weights of a population of neural networks multiple times during training, leading to performance gains.
%
On the other hand, works that have focused on providing feature alignment methods to be able to merge models in settings in which LMC is not trivial have mainly done so for 2 models at the time
%or for populations of simpler models such as MLPs trained on MNIST
\citep{singh-jaggi2020_OT-fusion, ainsworth2023_git-rebasin, pena2023_sinkhorn-rebasin, jordan2023repair}. An exception to this is Git Re-Basin \citep{ainsworth2023_git-rebasin} which proposes a ``Merge Many'' algorithm for merging a set of multiple models by successively aligning each model to the average of all the other models. However, results obtained with this method, which they use to merge up to 32 models, are relegated to the appendix and only concern the very simple set-up of MLPs on MNIST. \cite{singh-jaggi2020_OT-fusion} also consider merging multiple models but either in a similarly simple set-up, i.e. 4 MLPs trained on MNIST, or they fine-tune the resulting model after merging up to 8 VGG11 models trained on CIFAR100.
%
We extend this line of work to more challenging settings, using more complex model architectures, we report the merged models accuracies directly without fine-tuning and make this a key focus in our work.
\vspace{-5pt}
\paragraph{Model merging beyond permutations} We note that the two model merging methods based on optimal transport \cite{singh-jaggi2020_OT-fusion, pena2023_sinkhorn-rebasin} can also align models beyond permutations. However, in \cite{singh-jaggi2020_OT-fusion} this only happens when the two models being merged have different numbers of neurons at each layer. When the models have the same number of neurons the alignment matrix found by their method is a permutation, as such the majority of their results are with permutations. The method proposed by \cite{pena2023_sinkhorn-rebasin} isn't constrained to finding binary permutation matrices but binarity is still encouraged through the addition of an entropy regularizer. Furthermore, our CCA based method is different in nature from both of these since it is not inspired by optimal transport theory.
\vspace{-5pt}
% \paragraph{CCA in deep learning}
% Canonical Correlation Analysis is a very popular statistical method used in many fields of science \cite{DeBie2005}. In the context of deep learning, CCA has been used to align and compare learned representations in deep learning models \cite{raghu2017_svcca, morcos2018_insights}, a task which is very similar to the feature matching considered by model merging algorithms.

==> archive/s3_background.tex <==
\vspace{-2pt}
\section{Using CCA to merge models}\label{s:cca_merge_theory}
\vspace{-3pt}
\subsection{Merging Models: Problem Definition}
\vspace{-5pt}
Let $\mathcal{M}$ denote a standard MLP and layer $L_i\in\mathcal{M}$ denote a linear layer with a $\sigma=\text{ReLU}$ activation function, weights $W_i\in\mathbb{R}^{n_i\times n_{i-1}}$ and bias $b_i\in\mathbb{R}^{n_i}$. Its input is the vector of embeddings from the previous layer $x_{i-1}\in\mathbb{R}^{n_{i-1}}$ and its output can be described as:
%
\[x_i = \sigma(W_ix_{i-1}+b_i)\]
%
Consider two deep learning models $\mathcal{A}$ and $\mathcal{B}$ with the same architecture. Let $\{L_i^\mathcal{M}\}_{i=1}^N$ be the set of layers of model $\mathcal{M}\in\{\mathcal{A}, \mathcal{B}\}$ and let $X_i^\mathcal{M}\in\mathbb{R}^{m\times n_i}$ denote the set of outputs of the $i$-th layer of model $\mathcal{M}$ in response to $m$ given inputs. Given the context, we assume $X_i^\mathcal{M}$ is centered so that each column has a mean of 0. We are interested in the problem of merging the parameters from models $\mathcal{A}$ and $\mathcal{B}$ in a layer-by-layer fashion. In practice, it is often easier to keep model $\mathcal{A}$ fixed and to find a way to transform model $\mathcal{B}$ such that the average of their weights can yield good performance.
%
Mathematically, we are looking for invertible linear transformations $T_i\in\mathbb{R}^{n_i\times n_i}$ which can be applied at the output level of model $\mathcal{B}$ layer $i$ parameters to maximize the ``fit'' with model $\mathcal{A}$'s parameters and minimize the interpolation error. The output of the transformed layer $i$ of $\mathcal{B}$ is then:
\[x_i^\mathcal{B} = \sigma(T_iW_i^\mathcal{B}x_{i-1}^\mathcal{B}+T_ib^\mathcal{B}_i)\]
We therefore also need to apply the inverse of $T$ at the input level of the following layer's weights to keep the flow of information consistent inside a given model:
%
\[x_{i+1}^\mathcal{B} = \sigma(W_{i+1}^\mathcal{B}T_i^{-1}x_{i}^\mathcal{B}+b^\mathcal{B}_{i+1})\]
%
Depending on the model architecture, it might not be necessary to compute transformations after each single layer, for example, skip connections preserve the representation space, and the last layers of models are already aligned by the training labels. Therefore we refer to the specific layers in a network where transformations must be computed as ``merging layers''. After finding transformations $\{T_i\}_{i=1}$ for every merging layer in the network we can merge the two model's parameters:
%
\begin{equation}\label{eq:merging}
    W_i = \frac{1}{2}(W_i^\mathcal{A} + T_iW_i^\mathcal{B}T^{-1}_{i-1})
\end{equation}
%
\paragraph{Merging multiple models} In the case where multiple models are being merged there is a simple way of extending any method which aligns features between two models to the multiple models scenario. Suppose we have a set of models $\{\mathcal{M}_i\}_{i=1}^n$ which we want to merge. We can pick one of them, say $\mathcal{M}_j$ for $1\leq j\leq n$, to be the \emph{reference model}. Then we can align the features of every other model in the set to those of the reference model and average the weights. While this ``all-to-one'' merging approach is quite \textcolor{red}{straightforward} it seems to work well in practice.

\subsection{Background on Canonical Correlation Analysis}
Canonical Correlation Analysis (CCA) is a statistical method aiming to find relations between two sets of random variables. Suppose we have two datasets $X$ and $Y$ both of sizes $n\times d$, where $n$ is the number of instances or samples, and $d$ is the dimensionality or the number of features. Further, suppose that these datasets are centered so that each column has a mean of 0. 
%
CCA aims to find vectors $p_X$ and $p_Y$ in $\mathbb{R}^d$ such that the projections $Xp_X$ and $Yp_Y$ have maximal correlation and norm 1.

Let $S_{XX}=X^{\top}X$, $S_{YY}=Y^{\top}Y$ and $S_{XY}=X^{\top}Y$ denote the scatter matrix of $X$, the scatter matrix of $Y$ and the cross-scatter matrix of $X$ and $Y$ respectively. In practice, it is possible to use the respective covariance matrix which is simply $C=\frac{1}{n-1}S$ as it will yield the same solution vectors up to multiplication by a constant. The main optimization objective of CCA can be written as:
%
\begin{align*}
    p_X, p_Y &= \argmax\limits_{p_X, p_Y} p_X^\top S_{XY} p_Y\\
    & \text{s.t.}\quad \|Xp_X\|^2 = p_X^\top S_{XX} p_X = 1,\quad \|Yp_Y\|^2 = 1
\end{align*}
%
Formulating this as an ordinary eigenvalue problem and making it symmetric by a change of variable allows us to find the whole set of solutions as the vectors in $P_X$ and $P_Y$:
% This can be formulated as an ordinary eigenvalue problem:
% %
% \begin{align*}
%     \begin{pmatrix}
%         \mathbf{0} & S_{XX}^{-1}S_{XY}\\
%         S_{YY}^{-1}S_{YX} & \mathbf{0}
%     \end{pmatrix}
%     \begin{pmatrix}
%         p_X\\
%         p_Y
%     \end{pmatrix} = \lambda
%     \begin{pmatrix}
%         p_X\\
%         p_Y
%     \end{pmatrix}
% \end{align*}
% %
% Which can be made symmetric by introducing the vectors $v_X = S_{XX}^{1/2}p_X$ and $v_Y = S_{YY}^{1/2}p_Y$. 
% %
% \begin{align*}
%     \begin{pmatrix}
%         \mathbf{0} & S_{XX}^{-1/2}S_{XY}S_{YY}^{-1/2}\\
%         S_{YY}^{-1/2}S_{YX}S_{XX}^{-1/2} & \mathbf{0}
%     \end{pmatrix}
%     \begin{pmatrix}
%         v_X\\
%         v_Y
%     \end{pmatrix} = \lambda
%     \begin{pmatrix}
%         v_X\\
%         v_Y
%     \end{pmatrix}
% \end{align*}
% %
% We can then find $v_X$ and $v_Y$ as being the left and right singular vectors of $S_{XX}^{-1/2}S_{XY}S_{YY}^{-1/2}$ respectively. The projection vectors are therefore $p_X = S_{XX}^{-1/2}v_X$ and $p_Y = S_{YY}^{-1/2}v_Y$. If we want the dimensionality of the common space to be the same as the embedding spaces we can use the whole set of left and right singular vectors of $S_{XX}^{-1/2}S_{XY}S_{YY}^{-1/2}$:
%
\begin{align*}
    U, S, V^\top &= \text{SVD}(S_{XX}^{-1/2}S_{XY}S_{YY}^{-1/2})\\
    P_X &= S_{XX}^{-1/2}U \quad \text{and} \quad P_Y = S_{YY}^{-1/2}V 
\end{align*}
%
For more details we direct the reader to \cite{DeBie2005} from which this section was inspired.

\subsection{CCA Merge: Merging models with CCA}
To merge models using CCA we simply apply the CCA algorithm to the two sets of activations $X_i^\mathcal{A}$ and $X_i^\mathcal{B}$ to get the corresponding projection matrices $P_i^\mathcal{A}$ and $P_i^\mathcal{B}$. Using the framework described above of matching model $\mathcal{B}$ to model $\mathcal{A}$, which is consistent with past works, we can define $T_i=\nolinebreak \left(P_i^\mathcal{B}{P_i^\mathcal{A}}^{-1}\right)^\top$. The transpose here is to account for the fact that $T_i$ multiplies $W_i$ on the left while the $P_i$s were described as multiplying $X_i$ on the right. This transformation can be thought of as first bringing the activations of model $\mathcal{B}$ into the common, maximally correlated space between the two models by multiplying by $P_i^\mathcal{B}$ and then applying the inverse of $P_i^\mathcal{A}$ to go from the common space to the embedding space of $\mathcal{A}$. The averaging of the parameters of model $\mathcal{A}$ and transformed $\mathcal{B}$ can then be conducted following Eq.~\ref{eq:merging}.


==> archive/z0_additional_text.tex <==
\section{Discussion}
Past works have focused almost exclusively on merging only pairs of models. While some papers discuss the possibility of merging multiple models, the proposed method is simply to apply the 2 model merging method iteratively to align all models to a single, reference model, and then to average all models. While this works to some extent in practice and is also what we do with CCA merging, it would be interesting to explore methods that are inherently made to merge multiple models all at once.

Our method is somewhat unsymmetric, merging model X to model Y destroys some of the information from model X. Despite this we perform better than the other methods we compare to.

\paragraph{Merging spaces} When the model architecture is such that the information flows sequentially from input layer to output layer, as is the case for MLPs or VGGs, a transformation needs to be computed after each layer. However, when the architecture is more complex, as is the case for ResNets for example, the transformations are not necessarily computed at each layer, rather they are computed whenever there is a change in the representation space. We refer to these specific points in a network as ``merging'' or ``alignment'' spaces. For example, blocks containing skip connections preserve the same representation space since the output space is forced to be consistent with the input one by the skip connections. The convolutional layers inside the block on the other hand can transform the representation spaces an therefore transformations need to be computed after those.

\paragraph{A note on merging in the common space}
Given that CCA naturally finds a space which maximally correlates the activations of both models being merged it is natural to think of merging the models in this common space. This would be done by transforming the parameters of model $\mathcal{A}$ with the found transformations $\{W_i^\mathcal{A}\}_{i=1}^{N-1}$ and transforming the parameters of model $\mathcal{B}$ with transformations $\{W_i^\mathcal{B}\}_{i=1}^{N-1}$ and then averaging the transformed parameters. We have tried this with no success. We hypothesize that the reason this way of merging fails is that the common representation space found by CCA is not fit to work with ReLU activation functions. The following paragraph provides a justification for this hypothesis.

For the pre-activations to remain informative after the application of ReLU, all the important information needs to be in the orthant (high-dimensional analog of the quadrant in the plane) of the pre-activation space corresponding to all variables having greater values than zero. That way important information is preserved by the ReLU function and only un-important information, which can be found in the other orthants with some variables having negative values, get squashed to 0. There is no inherent reason for the common space found by CCA to keep important information only in the positive orthant, rather it likely spreads it across all orthants. As the dimensionality of the space increases, the ratio between the volume of the positive orthant and the rest of the volume of the space decreases exponentially, in 1D the positive part of the line represents half of the space, in 2D the positive quadrant represents one quarter of the plane, in 3D the positive orthant represents one eighth of the space, etc. Therefore, given the typical high dimensionality of ANN embedding spaces it is probable that only a small fraction of the important information is kept in the positive orthant and thus preserved after applying the ReLU activation, on the other hand the rest of the information is getting at least partially squashed to 0.

\paragraph{Why CCA Merge destroys in part the model being aligned}
It is well known that artificial neural networks are invariant to permutations. Permuting the order of the neurons at a given layer equivalently permutes the pre-activations, the activations and any other commonly used operations in ANNs which are applied element-wise.
%
On the other hand, when considering linear combinations of features, as we do for CCA Merge, the weights of a given layer are combined as dictated by the found transformation $T$, recall the two equations:
\[x_i^\mathcal{B} = \sigma(T_iW_i^\mathcal{B}x_{i-1}^\mathcal{B}+T_ib^\mathcal{B}_i)\]
\[x_{i+1}^\mathcal{B} = \sigma(W_{i+1}^\mathcal{B}T_i^{-1}x_{i}^\mathcal{B}+b^\mathcal{B}_{i+1})\]
Since $T$ here linearly combines features and is not simply a change in the order of those features, applying a non-linear activation function element-wise will affect the activations themselves, which will no longer have the same numerical values as the un-transformed ones (albeit possibly in a different order). Therefore, when applying the inverse transformation $T^{-1}$ to these activations we are not able to reconstruct the exact representations of the original models.
Additionally, since the inverse transformation $T^{-1}$ is only applied at the level of the weights of the following layer, it receives the activations post activation function and no longer allows to retrieve the exact same.

Suppose we are trying to merge two models $\mathcal{A}$ and $\mathcal{B}$ so we align model $\mathcal{B}$ to model $\mathcal{A}$ by applying the found transformations at relevant layer. We denote the aligned model $\mathcal{B}$ by $\mathcal{B}'$, i.e. model $\mathcal{B}$ after applying all the transformations $\{T_i\}$ and their inverses $\{T^{-1}_i\}$ to the relevant layers. If the transformations are permutations, then $\mathcal{B}$ and $\mathcal{B}'$ are equivalent and represent the same mathematical function, modulo permutations of their internal representations. If on the other hand the transformations are not permutations, but rather linear combinations as it is the case for CCA Merge, then the two models are no longer equivalent. 

% \begin{table}[t]
% \caption{VGG11/CIFAR10-Logits whole dataset 2 models averaging accuracies}
% \label{t:resnet20_cifar100_none}
% \begin{center}
% \begin{tabular}{l|l l l l}
%             Widths & x1 & x2 & x4 & x8\\
%             \hline
%             Base models avg. & 87.24 $\pm$ 0.23\% & 87.44 $\pm$ 0.70 \% & 87.85 $\pm$ 0.25\% & 87.93 $\pm$ 0.50\%\\
%             Ensemble & 90.47 $\pm$ 0.12\% & 90.42 $\pm$ 0.22\% & 90.81 $\pm$ 0.09\% & 90.75 $\pm$ 0.20\%\\
%             \hline
%             Direct averaging & 10.00 $\pm$ 0.01\% & 10.00 $\pm$ 0.01\% & 10.00 $\pm$ 0.01\% & 10.00 $\pm$ 0.01\%\\
%             Permute & 15.44 $\pm$ 2.50\% & 16.73 $\pm$ 3.77\% & 24.55 $\pm$ 1.58\% & 19.99 $\pm$ 3.48\%\\
%             ZipIt! & 12.41 $\pm$ 2.60\% & - & - & - \\
%             \hline
%             \rowcolor{BrightGreen}
%             CCA & 80.23 $\pm$ 2.16\% & 78.14 $\pm$ 1.29\% & 84.44 $\pm$ 0.93\% & 82.38 $\pm$ 2.37\%\\
%         \end{tabular}
% \end{center}
% \end{table}

% [INTERPOLATION PLOTS, ONLY 2 SPLITS]

% [TABLES WITH RESULTS, ONLY 2 SPLITS]

% \begin{table}[t]
% \caption{ResNet20/CIFAR100 unbalanced subsets model averaging accuracies}
% \label{t:resnet20_cifar100_unbalanced}
% \begin{center}
% \begin{tabular}{l|l l l l}
%             Widths & x1 & x2 & x4 & x8\\
%             \hline
%             Base models & 52.61 $\pm$ 1.84\% & 56.78 $\pm$ 1.96 \% & 58.74 $\pm$ 1.93\% & 59.98 $\pm$ 1.80\%\\
%             Ensemble & 64.68 $\pm$ 0.76\% & 69.92 $\pm$ 0.75\% & 72.18 $\pm$ 0.67\% & 73.77 $\pm$ 0.44\%\\
%             \hline
%             Direct averaging & 1.48 $\pm$ 0.17\% & 3.12 $\pm$ 0.49\% & 7.03 $\pm$ 0.49\% & 20.55 $\pm$ 3.07\%\\
%             Permute & 20.66 $\pm$ 0.87\% & 39.05 $\pm$ 0.42\% & 51.55 $\pm$ 0.86\% & 58.45 $\pm$ 1.76\%\\
%             CCA & 24.46 $\pm$ 320\% & 44.59 $\pm$ 1.80\% & 55.61 $\pm$ 0.63\% & 60.38 $\pm$ 1.68\%\\
%         \end{tabular}
% \end{center}
% \end{table}

% \begin{table}[t]
% \caption{ResNet20/CIFAR100-CLIP whole dataset 5 models averaging accuracies}
% \label{t:resnet20_cifar100_none}
% \begin{center}
% \begin{tabular}{l|l l l l}
%             Widths & x1 & x2 & x4 & x8\\
%             \hline
%             Base models avg. & 69.19 $\pm$ 0.22\% & 74.06 $\pm$ 0.19 \% & 77.23 $\pm$ 0.32\% & 78.73 $\pm$ 0.24\%\\
%             Ensemble & 76.53 $\pm$ 0.14\% & 79.55 $\pm$ 0.11\% & 81.54 $\pm$ 0.05\% & 82.24 $\pm$ 0.16\%\\
%             \hline
%             Direct averaging & 1.02 $\pm$ 0.12\% & 1.06 $\pm$ 0.23\% & 1.27 $\pm$ 0.10\% & 1.46 $\pm$ 0.11\%\\
%             Permute & 17.01 $\pm$ 2.31\% & 32.18 $\pm$ 0.77\% & 51.81 $\pm$ 0.53\% & 65.25 $\pm$ 0.24\%\\
%             Git Re-Basin & - & 44.69 $\pm$ 1.04\% & 59.67 $\pm$ 0.32\% & 67.21 $\pm$ 0.14\%\\
%             Many Merge & - & 3.82 $\pm$ 0.66\% & 5.26 $\pm$ 0.44\% & 10.19 $\pm$ 0.53\%\\
%             ZipIt! & 14.51 $\pm$ 0.99\% & 33.68 $\pm$ 1.24\% & 50.93 $\pm$ 0.49\% & 62.89 $\pm$ 0.38\%\\
%             \hline
%             \rowcolor{BrightGreen}
%             CCA & 25.19 $\pm$ 0.63\% & 49.54 $\pm$ 0.46\% & 62.72 $\pm$ 1.01\% & 72.66 $\pm$ 0.14\%\\
%         \end{tabular}
% \end{center}
% \end{table}

% In Tables \ref{t:resnet20_cifar100_none} and \ref{t:resnet20_cifar100_unbalanced} we show our results for the ResNet20 models of different widths trained on the CIFAR100 whole dataset or on unbalanced splits of the datasets respectively. We can see that across all model widths and both data distribution scenarios aligning model features with CCA leads to a smaller loss in accuracy when averaging the two aligned models than using permutations. Directly averaging the weights of the models without any kind of feature matching transformations yields very poor results as expected.
% %
% These results suggest that indeed looking for one-to-one mappings between neurons might be too restrictive since it does not capture more complex interactions between features of different models. The performance of CCA merging here suggests that computations conducted by some neurons in one network might be distributed across multiple neurons in another model.
